Dehn surgeries and rational homology balls

We consider the question of which Dehn surgeries along a given knot bound rational homology balls. We use Ozsv\'ath and Szab\'o's correction terms in Heegaard Floer homology to obtain general constraints on the surgery coefficients. We then turn our attention to the case of integral surgeries, with particular emphasis on positive torus knots. Finally, combining these results with a lattice-theoretic obstruction based on Donaldon's theorem, we classify which integral surgeries along torus knots of the form $T_{kq\pm 1,q}$ bound rational homology balls.

==> 2and3.tex <==

\section{$r/2$--surgeries}

\begin{lemma}\label{l:Lq2}
The correction term $d(L(m^2,m^2-2),i)$ is integer if and only if $i\equiv \frac{m^2+1}2 \pmod m$. More precisely, if $i = i_h = \frac{m^2+1}2 - hm$ with $-\frac{m-1}2\le h \le \frac{m-1}2$, then
\[\displaystyle
d(L(m^2,m^2-2),i) = \left\{\begin{array}{ll}
\displaystyle\frac{h^2-1}2 & {\rm if}\,h\,{\rm odd}\\
\displaystyle\frac{h^2}2 & {\rm if}\,h\,{\rm even}
\end{array}\right.
\]
\end{lemma}

\begin{proof}
This is a straightforward consequence of \cref{e:Lrecursion}.
\end{proof}

\begin{lemma}\label{l:Vq2}
Let $p,q$ be coprime positive integers, with $p=m^2$. If $S^3_{p/q}(K)$ bounds a rational homology ball, then
\begin{align*}
&4V_{({m^2-3-2hm})/4}(K) = h^2-1,\,{\rm if}\,h\,{\rm odd},\\
&4V_{({m^2-3-2hm-2})/4}(K) = h^2,\,{\rm if}\,h\,{\rm even}.
\end{align*}
\end{lemma}

\begin{proof}
If we apply \cref{e:NiWu} with $q = 2$ and $i<p/2$ we obtain:
\begin{equation}\label{e:NiWu2}
d(S^3_{p/2}(K),i) = -2V_{\lfloor i/2\rfloor}(K) + d(S^3_{p/2}(O),i).
\end{equation}
It now follows from \cref{l:Lq2} that for $h=0,\dots,\frac{m-1}2$ we have
\begin{equation}\label{e:fracparts}
\left\lfloor \frac{\frac{m^2-3}2-hm}2 \right\rfloor = \left\{\begin{array}{ll}
\displaystyle\frac{m^2-3-2hm}4 & {\rm if}\,h\,{\rm odd}\\
\displaystyle\frac{m^2-3-2hm-2}4 & {\rm if}\,h\,{\rm even}.
\end{array}\right.
\end{equation}
The desired computation is obtained by combining \cref{e:NiWu2} and \cref{e:fracparts}.
\end{proof}

\begin{prop}
If $S^3_{m^2/2}(K)$ bounds a rational homology ball and $m\ge 3$, and $\nu = \nu^+(K)$, then
\[
1+\sqrt{4\nu+5} \le m < 2+\sqrt{4\nu+9}.
\]
If $m=1$, then $\nu = 0$.
\end{prop}

\begin{proof}
The case $m=1$ is easier, since in that case the only correction term of $S^3_{1/2}(K)$ is $-2V_0(K)$; if $S^3_{1/2}(K)$ bounds a rational homology ball, then its correction term vanishes, and hence $\nu = 0$.

Suppose now $m\ge 3$. Analogously to what we have done in the previous section, observe that $\frac{m-1}2\ge 1$, and setting $h=1$ in \cref{l:Vq2} above gives the minimal integer $i$ such that $d(L(m^2,m^2-2),i)$ vanishes.
If $S^3_{m^2/2}(K)$ bounds a rational homology ball, then the corresponding $V_i(K)$ has to vanish, too. In particular, by the definition of $\nu$ we obtain
\[
\frac{m^2-3-2m}4 \ge \nu,
\]
from which the left-hand side inequality readily follows.

If now $m=3$, the right-hand side inequality is automatically satisfied; if $m>3$, $\frac{m-1}2\ge 2$, and setting $h=2$ in \cref{l:Vq2} gives an integer $i$ such that $V_i(K)$ does not vanish, since the corresponding correction term of $L(m^2,m^2-2)$ is nonzero, hence
\[
\frac{m^2-3-4m-2}4 < \nu,
\]
from which one obtains the right-hand side inequality.
\end{proof}

\begin{rem}
In particular, since $2+\sqrt{4\nu+9} - (1+\sqrt{4\nu+5}) < 2$, there is at most one odd integer in the range, and for infinitely many values of $\nu$ there are no odd integers at all.
\end{rem}

\begin{prop}
Let $p,q$ be coprime integers such that $p>9q$. Then $S^3_{m^2/2}(T_{p,q})$ never bounds a rational homology ball.
\end{prop}

\begin{proof}
Let $\nu = \nu^+(T_{p,q}) = \frac{(p-1)(q-1)}2$. Observe that if $\nu \ge 25$, then $m$ is at least $13$; since $m$ is odd, it is enough to show that the lower bound given by the proposition above is larger than 11:
\[
11 < 1 + \sqrt{25\cdot4 + 5} \le 1+\sqrt{4\nu+5} \le m.
\]
Notice also that if $p>9q$, then $\nu < 25$ only if $q=2$ and $p\le 49$. We will deal with this case later.

Hence, As in the proof of \cref{p:pvs9q}, if $p>9q$ the last nine gaps in the semigroup generated by $p,q$ are $g_9 < \dots < g_1$, where $g_k = (q-1)p-kq$. Since $m \ge 13$, we can look at the four correction terms labelled $i_h$, for $h=2,3,5,6$, we see that
\[
i_6 < g_9 < g_7 \le i_5,\quad g_3 < i_3 < i_2 \le g_1,
\]
from which
\begin{align*}
\frac{m-1}2 =& \frac{m^2-3-10m-2}4 - \frac{m^2-3-12m}4 > 2q,\\
\frac{m-1}2 =& \frac{m^2-3-4m-2}4 - \frac{m^2-3-6m}4 < 2q
\end{align*}
hence yielding a contradiction.

As for the case $q=2$, notice that $m\ge 7$ if $p\ge7$ (and in particular if $p>18 = 9q$), and we can still use the information coming from $i_2$ and $i_3$, hence the inequality $m<2q = 4$ still holds. But this contradicts the fact that $m\ge 7$.
\end{proof}

In fact, the only two $m^2/2$--surgeries along a torus knot $T_{2,2k+1}$ that could bound are $S^3_{25/2}(T_{3,2})$ and $S^3_{25/2}(T_{5,2})$, for which the correction terms do not give any obstruction.

However, the former has been shown not to bound in {\color{red}somewhere above}. The latter does not bound, either: it is the boundary of the negative-definite plumbing {\color{red} disegnarlo: è un $D_8$ con due 3 aggiunti ad una gamba corta e ad una lunga.},
which can easily be shown not to be embeddable in $\Z^{10}$.

\section{$r/3$--surgeries}

\begin{lemma}
The correction term $d(L(m^2,m^2-3),i)$ is integer if and only if $i = i_h = \frac{m(m-3)}2 + 1 - hm$ with $-\frac{m+1}2\le h \le \frac{m-3}2$; more precisely, in this case
\[\displaystyle
d(L(m^2,m^2-3),i) = \left\{\begin{array}{ll}
\displaystyle\frac{h(h+3)}3 & {\rm if}\,h \equiv 0 \pmod 3\\
\displaystyle\frac{(h+1)(h+2)}3 & {\rm if}\,h\not\equiv 0 \pmod 3
\end{array}\right.
\]
\end{lemma}

\begin{proof}
This is a straightforward computation from Ozsv\'ath and Szab\'o's recursion for correction terms of lens spaces.
\end{proof}

\begin{rem}
Observe that since $\gcd(m,3)=1$, then $m(m-3) \equiv m^2 \equiv 1 \pmod 3$, hence $i_0 \equiv 0\pmod 3$, and in particular $i_h \equiv 0\pmod 3$ if and only if $h\equiv 0 \pmod 3$.
\end{rem}

Analogously as above, we obtain that if $S^3_{m^2/3}(K)$ bounds a rational homology ball, then for each $i\le m^2/2$ of the form above we have
\[
V_{\lfloor i/3\rfloor}(K) = \frac{d(L(m^2,m^2-3),i)}2,
\]
and in particular, for $i\equiv 0\pmod 3$ (that is, for $h\equiv 0\pmod 3$), we obtain
\[
V_{i/3} = \frac{h(h+3)}6,
\]
while for $i\not\equiv 0 \pmod 3$
\[
V_{\lfloor i/3\rfloor} = \frac{(h+1)(h+2)}6.
\]
where the index is $(i-2)/3$ if $hm\equiv 1\pmod 3$ and $(i-1)/3$ otherwise.

\begin{prop}
Let $K$ be a knot in $S^3$ with $\nu^+(K) = \nu$. If $S^3_{m^2/3}(K)$ bounds a rational homology ball and $m\ge2$, then
\[
\frac{3+\sqrt{1+24\nu}}2 \le m < \frac{5+\sqrt{25+24\nu}}2.
\]
If $m=1$ or $m=2$, then $\nu = 0$.
\end{prop}

\begin{proof}
The case $m=1$ follows as in the previous section. If $m=2$, we can still consider the correction term associated to the $0$-th \spinc structure, which shows that $V_0(K) = 0$, hence $\nu(K) = 0$. The right-hand side inequality is automatically satisfied.

If $m\ge4$ we plug in $i_0$ (which is now positive): since $V_{i_0/3}=0$, then $\frac{i_0}3\ge\nu$ and the left-hand inequality follows. Notice that if $m=4$, the right-hand side inequality is automatically satisfied.

If $m\ge 5$, we plug in $i_1$ (which is positive), and notice that
\[
\left\lfloor \frac{i_1}3\right\rfloor = \frac{m(m-3)+1}3 - \left\lfloor \frac{m}3\right\rfloor - 1 \ge \frac{m^2-5m}6.
\]
Since $V_{\lfloor {i_1}/3\rfloor} (K) = 1$, then 
\[
\frac{m^2-5m}6 \le \left\lfloor \frac{i_1}3\right\rfloor \le \nu,
\]
from which we obtain the right-hand side inequality.
\end{proof}

\begin{prop}
If $S^3_{m^2/3}(T_{p,q})$ bounds a rational homology ball and $q\ge 3$, then $p<6q$.
\end{prop}

\begin{proof}
As in the previous subsections, we just make the following observations. Call $n = \lfloor m/3\rfloor$, $j_k = \lfloor i_k/3\rfloor$, and $V(j) = V_j(T_{p,q})$ as shorthand notations. As above, call $g_7 < \dots < g_1 = pq-p-q$ the gaps of the semigroup.

Suppose that $p>6q$: as discussed above, $g_k = g_1 - (k-1)q$ for $k=1,\dots,7$. If now $q \ge 3$, then $\nu \ge 18$, and from the proposition above it follows that $m\ge \frac{3+\sqrt{1+24\cdot 18}}2 > 11$, hence $m\ge 13$ (since it needs to be coprime with 3), hence $j_5$ is nonnegative.

Since $V(j_1) = 1$ and $V(j_2) = 2$, then $g_4 \ge j_3 < j_1 < g_1$, hence $j_1-j_3 < 3q$. Notice that $j_1 - j_3$ is $2n$ if $m\equiv1\pmod 3$ and is $2n+1$ if $m\equiv 2 \pmod 3$.

Analogously, since $V(j_3) = 3$ and $V(j_5) = 7$, we get that $j_5 < g_7 < g_4 \le j_3$, hence $j_3-j_5 > 3q$. Notice that now $j_3-j_5$ is $2n+1$ if $m\equiv 1\pmod 3$ and it is $2n+2$ if $m\equiv 2\pmod 3$.

In particular, in either case we get a contradiction with the above inequality, since the two read
\[
\begin{array}{ll}
2n < 3q < 2n+1 & {\rm if}\, m\equiv 1 \pmod 3,\\
2n+1 < 3q < 2n+2 & {\rm if}\, m\equiv 2 \pmod 3.
\end{array}\qedhere
\]
\end{proof}

Only the cases when $q = 2$ and $\frac{p-1}2 = \nu(T_{2,p}) < 18$ are left to consider, since the argument above applies whenever $\nu(T_{p,q}) \ge 18$. If $p\ge 7$, the first proposition above implies that $m\ge 7$, which in turn means that $i_2\ge 0$, hence we can look at $i_1$ and $i_2$, and using the same inequality of the second proposition above we see that $m<3q = 6$, hence yielding a contradiction.

This leaves three cases: $S^3_{16/3}(T_{3,2})$, $S^3_{25/3}(T_{3,2})$ and $S^3_{25/3}(T_{5,2})$. The latter, however, is obstructed by the correction terms, since
\[
d(S^3_{25/3}(T_{5,2}), 6) = -d(L(25,3),6)-2V_1(T_{5,2}) = 0-2 \neq 0.
\]
{\color{red} la prima borda, perch\'e si vede dal diagramma di chirurgia (in forma canonica, \`e stellato con 3 nel vertice centrale e tre gambe: un 2---2 e due 2); nel secondo caso non borda, perch\'e [9,2,2] = 25/3 ``non si immerge iniettivamente''.}


